Minimum pricing or volumetric taxation? Quantity, quality and competition effects of price regulations in alcohol markets

Reforming alcohol price regulations in wine-producing countries is challenging, as current price regulations reflect the alignment of cultural preferences with economic interests rather than public health concerns. We evaluate and compare the impact of counterfactual alcohol pricing policies on consumer behaviors, firms, and markets in France. We develop a micro-founded partial equilibrium model that accounts for consumer preferences over purchase volumes across alcohol categories and over product quality within categories, and for firms' strategic price-setting. After calibration on household scanner data, we compare the impacts of replacing current taxes by ethanol-based volumetric taxes with a minimum unit price (MUP) policy of 0.50 Euro per standard drink. The results show that the MUP in addition to the current tax outperforms a tax reform in reducing ethanol purchases (-15% vs. -10% for progressive taxation), especially among heavy drinking households (-17%). The MUP increases the profits of small and medium wine firms (+39%) while decreasing the profits of large manufacturers and retailers (-39%) and maintaining tax revenues stable. The results support the MUP as a targeted strategy to reduce harmful consumption while benefiting small and medium wine producers. This study provides ex-ante evidence that is crucial for alcohol pricing policies in wine-producing countries.

==> AppIndividualisation.tex <==

We now show how household-level variations in total alcohol purchases are individualized using a statistical technique proposed by \textcite{chesher_diet_1997}. This will produce relative variations in alcohol intake for types of individuals characterized by their age, their gender and their habitual level of consumption. These relative variations in total alcohol intake will feed an epidemiological model that will simulate the markovian transitions of the population between three states - healthy, ill and dead - in the spirit of the consumption-to-harms block of the Sheffield model \parencite{purshouse_modelling_2009,holmes_effects_2014,brennan_sheffield_2015}

From Step 2, we will get a household-specific policy impact on ethanol purchases for at-home consumption. We will then apply the individualization procedure proposed by \textcite{chesher_diet_1997} to compute individual-level effects for household members, according
to their socio-demographic profiles. We now describe this procedure.

\subsection{Statistical model of individualisation}

We let $e_{p}^{ah}$ be the consumption of alcohol $a$ for individual $p$ in household $h$, and we specify a model for individual consumption:
\begin{equation*}
	e_{p}^{ah}=\beta^{a} \left( D_{p}^{h}\right) +u_{p}^{ah}  \label{indiv cons}
\end{equation*}
with $D_{p}^{h}$ a set of individual and household characteristics that are associated with individual consumption, and $u_{p}^{ah}$ an individual-specific error term.

Total household consumption can be written as the sum of individual consumptions and equalled to household purchases $E^{ah}$ up to some household-specific error term:
\begin{equation*}
	E^{ah}=\displaystyle\sum_{p=1}^{P(h)}y_{p}^{ah}=\displaystyle\sum_{p=1}^{P(h)}\beta^{a} \left(D_{p}^{h}\right) +\xi^{ah}  \label{hhcons}
\end{equation*}
\noindent where $\xi^{ah}=\displaystyle\sum_{p=1}^{P(h)}u_{p}^{ah}+\epsilon^{ah}$ is an i.i.d. error-term with zero conditional mean,   and $P(h)$ is the number of individuals in household $h$. The additional error-term $\epsilon^{ah}$ accounts for wastes and consumption by guests. We assume that the latter is uncorrelated with the socio-demographic variables, so that on average total consumption by household members is effectively equal to their total purchases: 
\begin{align*}
				&\mathbb{E}\left(u_{p}^{ah}|D_{1}^{h},..,D_{P(h)}^{h}\right) =0  \label{Eq:orthog} \\
	and \quad		& \mathbb{E}\left(\epsilon^{ah}|D_{1}^{h},..,D_{P(h)}^{h}\right)=0 \nonumber \\
	\Rightarrow \quad & \mathbb{E}\left(\nu^{ah}|D_{1}^{h},..,D_{P(h)}^{h} \right) =0 \nonumber
\end{align*}
This allows to consistently identify the function $\beta^{a}()$.
\bigskip

Following Chesher (1997), we specify $\beta^{a}()$ as the multiplication of an individual function and a household function. We let $D_{p}^{h}=\left\lbrace D_{p},D^{h}\right\rbrace$:
\begin{equation}
	\beta^{a} \left(D_{p}^{h}\right)=f^{a}\left(D_{p}\right)g^{a}\left(D^{h}\right) \label{eq:indiv}
\end{equation}
$g^{a}\left(D^{h}\right)$ takes an exponential form $g^{a}\left(D^{h}\right)=\exp\left(\zeta^{a}D^{h}\right)$, while $f^{a}(D_{p})$ is specified as a linear sum of sex-specific age and education fixed effects. If we partition the population in $B$ age classes, and $O$ education classes, and if we note $n_{bo}^{Mh}$ and $n_{bo}^{Fh}$ respectively the number of males and females individuals in household $h$, for each age class $b$,and education class $o$, the model is:
\begin{equation}
	E^{ah}  =    \left[\displaystyle\sum_{b}  \displaystyle\sum_{o}\left(n_{bo}^{Mh}  \beta_{bo}^{aM} + n_{bo}^{Fh}  \beta_{bo}^{aF} \right)\right] \times\exp\left(\zeta^{a}D^{h}\right)+\xi^{ah}  \label{Eq:Indiv}
\end{equation}
\noindent where the parameters to be estimated are the $\beta$s and $\zeta$.

We decided to adjust for the following household variables $D^{h}$: city size (more/less than 20000 inhabitants), number of children in the household, average household consumption per adult in 2013 ($[0,1]$, $]1,2]$, more than $2$ standard drinks), the four KWP income categories, and a dummy indicating whether the household resides in a territory that is a high  producer of alcohol $a$.\footnote{The territories are administrative entities called \enquote{Departement}. The dummy equals 1 if the Departement of residence has more producers of alcohol $a$ than the French median (or producers of any alcohol when we individualise total alcohol purchases). We use the median because for some alcohol categories (such as Beers), there is no Departement
without producers.} Note that this set of variables includes the variables that have been used in the specification of the demand for alcohol quantities (either as control variables or for clustering the observations), and in the specifications of the market models. 
\bigskip

A few additional details about the assumptions underlying this model:
\begin{itemize}
	\item we consider that children (individuals less than 16 years old) have a null alcohol consumption,
	\item we do not have education effects for individuals aged between 16 and 24,
	\item we constrain the $\beta$s to be positive, in order to get positive predicted consumptions at the individual level,
\end{itemize}

\subsection{Prediction of the relative variation in individual consumption}\label{sec:simulindiv}

After the estimation of model \ref{Eq:Indiv}, we can predict individual consumption in a way that preserve household heterogeneity. We first use the estimates by alcohol category $a$ to compute the share of household consumption accruing to individual $p$:
\begin{equation}
	\eta_{p}^{ha} = \frac{\widehat{y_{p}^{ha}}}{\displaystyle\sum_{p=1}^{P(h)}\widehat{y_{p}^{ha}}}
\end{equation}
We then assume that the estimated share of alcohol
intake provided by category $a$ to individual $p$ in household $h$, $\eta_{p}^{ha}$, is left unaffected by the policy. Hence, the relative variation in
individual alcohol intake coming from the off-trade consumption of category
$a$ will be calculated as:
\begin{equation}
	\Delta e_{p}^{ah}=\eta_{p}^{ha}\Delta E_{ah} \label{Eq:IndivVar}
\end{equation}
\noindent where $\Delta E_{ah}$ has been calculated in Step 2.
This will finally yield the total variation in alcohol intake for individual $p$:
\begin{equation}
	\Delta e_{p}^{h}=\displaystyle\sum_{a}\left[\frac{e_{p}^{ha0}}{\sum_{a}e_{p}^{ha0}}\Delta e_{p}^{ah}\right] \label{Eq:IndivVar}
\end{equation}

Note that this quantity will vary between individuals according to the rich set of observable individual and household characteristics that can be found in the various models, especially age, gender, Kantar economic classes and household drinking habits in 2013. 

\subsection{Estimation results}

We estimate equation \ref{eq:indiv} in sample S4, using the corresponding household sampling weights ($\omega_{h}^{S4}$) as we want to get results in terms of consumption averaged over the year.\footnote{As S4 is extracted from the permanent panel, KWP provides a yearly weight for each household in addition to the period-specific weights.} The dependent variable in the models ($E^{ah}$) is thus total household purchases over a year on alcohol category $a$, expressed in terms of ethanol (see Section \ref{Sec:KWPFormula} for the formula).

Table \ref{tab:indivresults} present the main estimation results. The first column presents the results for total ethanol purchases, while the six remaining columns present the individualisation results by alcohol category. The models were estimated on the subsamples of households with non-null purchases. Some of the $\beta$s had missing standard errors due to  alow number of observations in the corresponding gender $\times$ age $\times$ education cells. We removed them sequentially from the specification. 

The estimated $\beta$s conform to prior knowledge regarding the socio-demographic characteristics of consumption patterns in France. Intakes are higher in men than in women for all alcohol categories except sparkling wines. The 35-54 years-old is the age category with the highest consumption levels, before the elderly (65 years-old and more). The education-consumption gradient is often hump-shaped, although there are variations by age, gender and alcohol categories. For instance, it is U-shaped for still wines and older males. 

The socio-demographic variables moderates the effects of individual characteristics (see the $\zeta$s). There is a negative income gradient for total ethanol intakes (first column, $\zeta_{IncX}$), but this hides considerable heterogeneity across alcohol categories. Lower-middle and lower class individuals consume more beers (third column). Upper-middle class individuals consumer less spirits than the upper-class ones. Lower class individuals drink less sparkling wines. As expected individuals in households that purchase more are predicted to consume more ($\zeta_{StddrinksX}$). Living in a residential area will less than 20,000 inhabitants, or having children under 16 years-old decrease predicted individual consumption.

\begin{landscape}
	\begin{center}
		\small
		\begin{longtable}{llllllll}
				\caption{Estimation of individualization coefficients (year 2014)}\label{tab:indivresults} \\
				\hline\hline
				&\multicolumn{1}{c}{Total}&\multicolumn{1}{c}{Ciders}&\multicolumn{1}{c}{Beers}&\multicolumn{1}{c}{Aperitifs}&\multicolumn{1}{c}{Spirits}&\multicolumn{1}{c}{Still W.}&\multicolumn{1}{c}{Sparkling W.}\\
				\hline
				\endhead
				$\beta^{M.}_{[25;35[,short} $ & 1635.432***&    4.632         &  452.382***&   24.046         &  848.221***&  569.791***&                  \\
				$\beta^{M.}_{[25;35[,medium}$  & 1868.436***&   22.850*  &  642.018***&  138.190***&  191.686***&  803.248***&  199.773***\\
				$\beta^{M.}_{[25;35[,long}$  & 1532.228***&   65.580***&  444.786***&   81.946         &  191.238         &  841.721***&   55.572         \\
				$\beta^{M.}_{[35;55[,short}$  & 1548.067***&   93.845***&  357.239***&  245.004***&  542.193***&  664.563***&   55.152*  \\
				$\beta^{M.}_{[35;55[,medium}$  & 1939.076***&   56.477***&  386.684***&  232.348***& 1030.667***&  662.689***&   95.166***\\
				$\beta^{M.}_{[35;55[,long}$  & 1774.634***&  115.543***&  318.871***&  182.872***& 1040.644***&  522.232***&  164.006***\\
				$\beta^{M.}_{[55;65[,short}$  & 2138.354***&   48.137***&  550.318***&  328.690***&  572.473***&  902.417***&  138.840***\\
				$\beta^{M.}_{[55;65[,medium}$  & 2066.875***&   84.166***&  430.982***&  222.280***&  538.147***& 1058.353***&  253.567***\\
				$\beta^{M.}_{[55;65[,long}$  & 1496.745***&   85.525***&  524.295***&  187.033***&  453.484***&  674.035***&  104.042         \\
				$\beta^{M.}_{[65;+\inf[,short}$  & 1851.686***&   73.376***&  242.567***&  210.166***&  538.010***&  955.378***&  101.802***\\
				$\beta^{M.}_{[65;+\inf[,medium}$  & 1764.210***&   87.051***&  273.010***&  225.098***&  465.789***&  903.196***&   99.191***\\
				$\beta^{M.}_{[65;+\inf[,long}$  & 2432.991***&   32.699         &  321.122***&  135.441***&  601.178***& 1496.654***&   26.893         \\
				$\beta^{F.}_{[25;35[,short}$  &  107.756         &    8.931         &  146.393***&   42.533         &  115.435         &                  &                  \\
				$\beta^{F.}_{[25;35[,medium}$  & 1053.714***&   36.160** &  173.840***&  151.283***&  512.533***&  252.822***&  256.999***\\
				$\beta^{F.}_{[25;35[,long}$  &  980.606***&   75.930***&  223.439***&  157.318***&  495.934***&  162.183         &  187.800***\\
				$\beta^{F.}_{[35;55[,short}$  & 1403.940***&                  &   45.889         &  181.646***&  615.746***&  511.426***&  159.617***\\
				$\beta^{F.}_{[35;55[,medium}$  & 1093.180***&   51.390***&   69.044** &   89.682***&  441.433***&  433.298***&  215.518***\\
				$\beta^{F.}_{[35;55[,long}$  & 1118.290***&   38.211** &  169.527***&   92.753** &   30.507         &  793.830***&   29.280         \\
				$\beta^{F.}_{[55;65[,short}$  &  940.164***&    5.186         &   91.298***&   66.658***&  194.188***&  500.877***&  262.159***\\
				$\beta^{F.}_{[55;65[,medium}$  & 1441.778***&   58.725***&  124.101***&  119.692***&  548.702***&  568.793***&  249.430***\\
				$\beta^{F.}_{[55;65[,long}$  & 2367.483***&   13.994         &  395.250***&  296.005***&  983.182***& 1007.551***&   73.749         \\
				$\beta^{F.}_{[65;+\inf[,short}$  & 1025.013***&   71.011***&  153.403***&  209.982***&  254.847***&  426.265***&  180.450***\\
				$\beta^{F.}_{[65;+\inf[,medium}$  & 1298.337***&   19.402         &   86.945** &  258.129***&  165.206***&  804.779***&  203.609***\\
				$\beta^{F.}_{[65;+\inf[,long}$  &  590.679***&   64.850** &   78.675         &  140.470** &  128.810         &  129.189         &  498.514***\\
				$\beta^{M.}_{[16;25[,.}$    & 1444.740***&                  &  177.434***&                  &  217.439***&  914.074***&  423.191***\\
				$\beta^{F.}_{[16;25[,.}$    &  707.348***&    2.006         &  120.908***&  144.595***&  465.993***&   32.270         &   67.240*  \\
				\hline
				\newpage
				\caption[]{(continued)}\\
				\hline
				$\zeta_{ResidLess20000}$&   -0.074***&   -0.266***&    0.001         &   -0.143***&    0.030         &   -0.142***&    0.210***\\
				$\zeta_{NbChildrenLess16}$&   -0.081***&   -0.147***&    0.135***&   -0.132***&   -0.128***&   -0.168***&   -0.066         \\
				$\zeta_{Stddrinks2}$&    1.197***&    0.475***&    0.761***&    0.733***&    1.131***&    1.219***&    0.717***\\
				$\zeta_{Stddrinks3}$&    2.169***&    0.703***&    1.458***&    1.171***&    2.143***&    2.310***&    1.571***\\
				$\zeta_{Inc2}$   &    0.017         &   -0.354***&    0.088         &    0.253***&   -0.162***&    0.125***&    0.023         \\
				$\zeta_{Inc3}$   &    0.088***&   -0.139         &    0.242***&    0.334***&    0.092*  &    0.092***&    0.114         \\
				$\zeta_{Inc4}$   &    0.217***&    0.353***&    0.241***&    0.295***&    0.175***&    0.375***&   -0.282** \\
				$\zeta_{RegProd}$&   -0.063***&    0.670***&    0.050         &   -0.044         &   -0.088***&    0.007         &   -0.207***\\
				\hline
				$N$     &     9815         &     3426         &     7813         &     5867         &     6887         &     8855         &     4734         \\
				$R^{2}$        &    0.743         &    0.251         &    0.360         &    0.328         &    0.454         &    0.575         &    0.287         \\
				\hline\hline
		\end{longtable}
		\begin{center}
		\begin{minipage}{1.2\textwidth}
			{\small \textit{Notes}: * $p<0.10$, ** $p<0.05$, *** $p<0.01$; $\beta^{g.}_{bo}$ coefficients for gender $g=M,F$,class age $b=[16;25[,[25,35[,[35;55[,[55,65[,[55,+\inf[$, and education class $o$= short (less than Baccalaureat),medium (Baccalaureat and short higher education), long (long higher education);$\zeta_D$ are coefficients of households variables  $D^{h}$; $StddrinksX$ with X=2,3 are indicator variables for the household habitual level of consumption in 2013, [1,2[ standard drinks/adult/day ($Stddrinks2$) or more than 2 standard drinks/adult/day ($Stddrinks3$); $IncX$ are dummy variables for the household income category, upper-middle ($Inc2$), lower-middle ($Inc3$), lower ($Inc4$); $Regprod$ is a dummy variable indicating whether the household lives in an alcohol-producing region (first column) or in a region producing the alcohol category (other columns).    }
		\end{minipage}
	\end{center}
	\end{center}
\end{landscape}

